Bringing Light Into the Dark: A Large-scale Evaluation of Knowledge Graph Embedding Models Under a Unified Framework

The heterogeneity in recently published knowledge graph embedding models' implementations, training, and evaluation has made fair and thorough comparisons difficult. In order to assess the reproducibility of previously published results, we re-implemented and evaluated 21 interaction models in the PyKEEN software package. Here, we outline which results could be reproduced with their reported hyper-parameters, which could only be reproduced with alternate hyper-parameters, and which could not be reproduced at all as well as provide insight as to why this might be the case. We then performed a large-scale benchmarking on four datasets with several thousands of experiments and 24,804 GPU hours of computation time. We present insights gained as to best practices, best configurations for each model, and where improvements could be made over previously published best configurations. Our results highlight that the combination of model architecture, training approach, loss function, and the explicit modeling of inverse relations is crucial for a model's performances, and not only determined by the model architecture. We provide evidence that several architectures can obtain results competitive to the state-of-the-art when configured carefully. We have made all code, experimental configurations, results, and analyses that lead to our interpretations available at https://github.com/pykeen/pykeen and https://github.com/pykeen/benchmarking

==> tables/ablation.tex <==
% skyline bytes
\input{tables/ablation/fb15k237_model_bytes_skyline}
\input{tables/ablation/kinships_model_bytes_skyline}
\input{tables/ablation/wn18rr_model_bytes_skyline}
\input{tables/ablation/yago310_model_bytes_skyline}

% % % skyline time
% \input{tables/ablation/fb15k237_training_time_skyline}
% \input{tables/ablation/kinships_training_time_skyline}
% \input{tables/ablation/wn18rr_training_time_skyline}
% \input{tables/ablation/yago310_training_time_skyline}

% best
\input{tables/ablation/best}


==> tables/ablation/best.tex <==
\begin{table}
\centering
\caption{Best configuration for each model in FB15k237}
\label{best_models_fb15k237}
\begin{tabular}{llllr}
\toprule
   Model &  Loss & Training Approach & Inverse Relations &  Hits@10 (\%) \\
\midrule
 ComplEx &   CEL &              LCWA &              True &       44.838 \\
   ConvE &  BCEL &              LCWA &              True &       49.212 \\
  ConvKB &   SPL &             sLCWA &             False &       32.261 \\
DistMult &   CEL &              LCWA &              True &       47.387 \\
   ERMLP &  BCEL &              LCWA &              True &       45.100 \\
    HolE &   CEL &              LCWA &              True &       42.225 \\
    KG2E &   SPL &              LCWA &              True &       45.501 \\
    MuRE &  BCEL &              LCWA &              True &       47.199 \\
     NTN &   SPL &             sLCWA &             False &       20.342 \\
   ProjE &  BCEL &              LCWA &              True &       41.616 \\
   QuatE &   CEL &              LCWA &              True &       46.166 \\
  RESCAL &   CEL &              LCWA &              True &       46.460 \\
  RotatE & NSSAL &             sLCWA &             False &       49.750 \\
      SE & NSSAL &             sLCWA &              True &       39.427 \\
  SimplE &   CEL &              LCWA &              True &       40.307 \\
  TransD &   MRL &             sLCWA &              True &       41.856 \\
  TransE &   MRL &             sLCWA &             False &       46.423 \\
  TransH &   MRL &             sLCWA &             False &       35.295 \\
  TransR &   CEL &              LCWA &              True &       39.187 \\
  TuckER &  BCEL &              LCWA &              True &       52.857 \\
      UM &   CEL &              LCWA &             False &        8.024 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{Best configuration for each model in Kinships}
\label{best_models_kinships}
\begin{tabular}{llllr}
\toprule
   Model &  Loss & Training Approach & Inverse Relations &  Hits@10 (\%) \\
\midrule
 ComplEx &   CEL &              LCWA &              True &       98.371 \\
   ConvE & NSSAL &             sLCWA &              True &       98.557 \\
  ConvKB & NSSAL &             sLCWA &              True &       97.067 \\
DistMult &   CEL &              LCWA &              True &       93.529 \\
   ERMLP &   SPL &             sLCWA &              True &       97.486 \\
    HolE &   CEL &              LCWA &              True &       93.715 \\
    KG2E &   MRL &             sLCWA &              True &       91.853 \\
    MuRE &   SPL &              LCWA &              True &       95.019 \\
     NTN &  BCEL &             sLCWA &              True &       93.622 \\
   ProjE &   SPL &             sLCWA &              True &       96.648 \\
   QuatE &   CEL &              LCWA &              True &       98.184 \\
  RESCAL &   SPL &             sLCWA &              True &       97.719 \\
  RotatE & NSSAL &             sLCWA &             False &       98.557 \\
      SE & NSSAL &             sLCWA &              True &       98.324 \\
  SimplE &  BCEL &             sLCWA &             False &       98.277 \\
  TransD &   CEL &              LCWA &              True &       45.205 \\
  TransE &   CEL &              LCWA &              True &       92.877 \\
  TransH &   CEL &              LCWA &              True &       52.048 \\
  TransR &   MRL &             sLCWA &             False &       73.324 \\
  TuckER &   SPL &              LCWA &              True &       98.603 \\
      UM &   SPL &              LCWA &              True &       11.313 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{Best configuration for each model in WN18RR}
\label{best_models_wn18rr}
\begin{tabular}{llllr}
\toprule
   Model &  Loss & Training Approach & Inverse Relations &  Hits@10 (\%) \\
\midrule
 ComplEx &   CEL &              LCWA &             False &       53.745 \\
   ConvE &   CEL &              LCWA &              True &       56.327 \\
  ConvKB & NSSAL &             sLCWA &              True &       42.083 \\
DistMult &   CEL &              LCWA &              True &       52.616 \\
   ERMLP &   SPL &             sLCWA &              True &       47.657 \\
    HolE &   CEL &              LCWA &             False &       50.017 \\
    KG2E &   SPL &              LCWA &             False &       52.035 \\
    MuRE &   SPL &              LCWA &              True &       57.900 \\
     NTN &   MRL &             sLCWA &             False &       31.857 \\
   ProjE &   CEL &              LCWA &              True &       51.727 \\
   QuatE &   CEL &              LCWA &             False &       55.010 \\
  RESCAL &   CEL &              LCWA &             False &       53.916 \\
  RotatE &  BCEL &              LCWA &              True &       60.089 \\
      SE &   SPL &             sLCWA &             False &       45.486 \\
  SimplE &   CEL &              LCWA &              True &       50.889 \\
  TransD &   MRL &             sLCWA &             False &       46.546 \\
  TransE &   SPL &              LCWA &             False &       56.977 \\
  TransH &   MRL &             sLCWA &             False &       48.170 \\
  TransR &   MRL &             sLCWA &             False &       42.510 \\
  TuckER &   CEL &              LCWA &              True &       56.088 \\
      UM &   SPL &              LCWA &             False &       44.887 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{Best configuration for each model in YAGO310}
\label{best_models_yago310}
\begin{tabular}{llllr}
\toprule
   Model &  Loss & Training Approach & Inverse Relations &  Hits@10 (\%) \\
\midrule
 ComplEx &  BCEL &             sLCWA &              True &       62.575 \\
  ConvKB &   SPL &             sLCWA &              True &       58.149 \\
DistMult &  BCEL &             sLCWA &             False &       55.580 \\
   ERMLP &  BCEL &             sLCWA &              True &       58.531 \\
    HolE &  BCEL &             sLCWA &             False &       60.177 \\
    MuRE &   SPL &             sLCWA &              True &       66.851 \\
   QuatE &   SPL &             sLCWA &              True &       60.709 \\
  RESCAL &   SPL &             sLCWA &              True &       54.045 \\
  RotatE & NSSAL &             sLCWA &              True &       63.077 \\
      SE & NSSAL &             sLCWA &              True &       29.757 \\
  TransD &   MRL &             sLCWA &             False &       35.397 \\
  TransE &   MRL &             sLCWA &              True &       49.217 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/ablation/fb15k237_model_bytes_skyline.tex <==
\begin{table}[H]
\centering
\caption{Pareto-optimal models for FB15k237 regarding Model Bytes and Hits@10}
\label{tab:skyline_fb15k237_model_bytes}
\begin{tabular}{llllrr}
\toprule
   Model & Loss & Training Approach & Inverse Relations & Model Bytes &  Hits@10 (\%) \\
\midrule
  TuckER & BCEL &              LCWA &               yes &     8.0 MiB &       52.857 \\
DistMult &  CEL &              LCWA &               yes &     3.7 MiB &       47.387 \\
  TransE &  SPL &              LCWA &                no &     3.6 MiB &       45.318 \\
      UM &  MRL &             sLCWA &                no &     3.5 MiB &        3.432 \\
      UM &  MRL &             sLCWA &               yes &     3.5 MiB &        3.305 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/ablation/kinships_model_bytes_skyline.tex <==
\begin{table}[H]
\centering
\caption{Pareto-optimal models for Kinships regarding Model Bytes and Hits@10}
\label{tab:skyline_kinships_model_bytes}
\begin{tabular}{llllrr}
\toprule
 Model & Loss & Training Approach & Inverse Relations & Model Bytes &  Hits@10 (\%) \\
\midrule
TuckER &  SPL &              LCWA &               yes &     1.0 MiB &       98.603 \\
RotatE &  MRL &             sLCWA &               yes &   154.0 KiB &       98.557 \\
RotatE &  MRL &             sLCWA &                no &   129.0 KiB &       98.324 \\
SimplE & BCEL &              LCWA &               yes &    77.0 KiB &       97.765 \\
 ProjE &  SPL &             sLCWA &               yes &    39.3 KiB &       96.648 \\
 ProjE &  SPL &             sLCWA &                no &    33.0 KiB &       94.600 \\
  HolE &  CEL &              LCWA &                no &    32.2 KiB &       88.873 \\
    UM &  SPL &              LCWA &               yes &    26.0 KiB &       11.313 \\
    UM &  SPL &             sLCWA &               yes &    26.0 KiB &        6.844 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/ablation/wn18rr_model_bytes_skyline.tex <==
\begin{table}[H]
\centering
\caption{Pareto-optimal models for WN18RR regarding Model Bytes and Hits@10}
\label{tab:skyline_wn18rr_model_bytes}
\begin{tabular}{llllrr}
\toprule
 Model & Loss & Training Approach & Inverse Relations & Model Bytes &  Hits@10 (\%) \\
\midrule
RotatE & BCEL &              LCWA &               yes &    79.3 MiB &       60.089 \\
RotatE &  SPL &              LCWA &               yes &    19.8 MiB &       58.328 \\
TuckER &  CEL &              LCWA &               yes &    11.9 MiB &       56.088 \\
  MuRE &  SPL &              LCWA &                no &    10.2 MiB &       55.489 \\
TransH &  MRL &             sLCWA &                no &     9.9 MiB &       48.170 \\
    UM &  SPL &              LCWA &               yes &     9.9 MiB &       44.682 \\
    UM &  SPL &             sLCWA &               yes &     9.9 MiB &       39.022 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/ablation/yago310_model_bytes_skyline.tex <==
\begin{table}[H]
\centering
\caption{Pareto-optimal models for YAGO310 regarding Model Bytes and Hits@10}
\label{tab:skyline_yago310_model_bytes}
\begin{tabular}{llllrr}
\toprule
   Model &  Loss & Training Approach & Inverse Relations & Model Bytes &  Hits@10 (\%) \\
\midrule
    MuRE &   SPL &             sLCWA &               yes &    61.1 MiB &       66.851 \\
  ConvKB & NSSAL &             sLCWA &                no &    30.1 MiB &       52.921 \\
DistMult &   SPL &             sLCWA &               yes &    30.1 MiB &       50.562 \\
  TransE &  BCEL &             sLCWA &                no &    30.1 MiB &       14.663 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/ablation_loss.tex <==
% Results Of Ablation Study For Loss Functions On FB15k-237 Based on the \ac{owa}
\begin{table*}[t]
\caption{Results of the Ablation Study for Loss Functions on FB15K-237 Based on the \ac{owa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Loss Functions On WN18RR Based on the \ac{owa}
\begin{table*}[t]
\caption{Results Of Ablation Study For Loss Functions On WN18RR Based on the \ac{owa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Loss Functions On Yago3-10 Based on the \ac{owa}
\begin{table*}[t]
\caption{Results Of Ablation Study For Loss Functions On YAGO3-10 Based on the \ac{owa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Loss Functions On NELL Based on the \ac{owa}
\begin{table*}[t]
\caption{Results Of Ablation Study For Loss Functions On NELL Based on the \ac{owa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

\subsection{Study: Ablation Study For Loss Function Based On \ac{lcwa}}

Similar to the study described in Section~\ref{ablation_loss_owa}, we examined the effect of the loss function on the model's performance.
The difference is that for this study the models were trained based on the LCWA.

% Results Of Ablation Study For Optimizers  On FB15k-237 Based On LCWA
\begin{table*}[t]
\caption{Results Of Ablation Study For Loss Functions On FB15k-237 Based on \ac{lcwa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Optimizers  On WN18RR Based On LCWA
\begin{table*}[t]
\caption{Results Of Ablation Study For Loss Functions On WN18RR Based On LCWA.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Optimizers  On Yago3-10 Based On LCWA
\begin{table*}[t]
\caption{Results Of Ablation Study For Loss Functions On Yago3-10 Based On LCWA.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Loss Functions On NELL Based On LCWA
\begin{table*}[t]
\caption{Results Of Ablation Study For Optimizers  On NELL Based On LCWA.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

\subsection{Study: Ablation Study For Optimizer Based on the \ac{owa}}\label{ablation_study_optimizer_owa}

In this study, we investigated the effect of the optimizer on the model's performance when trained based on the \ac{owa}.
To reduce the number of experiments, we focused on ADADELTA~\cite{zeiler2012adadelta} and Adam~\cite{kingma2014adam}. 

% Results Of Ablation Study For Optimizers  On FB15k-237 Based on the \ac{owa}
\begin{table*}[t]
\caption{Results Of Ablation Study For Loss Functions On FB15k-237 Based on the \ac{owa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Optimizers  On WN18RR Based on the \ac{owa}
\begin{table*}[t]
\caption{Results Of Ablation Study For Optimizers On WN18RR Based on the \ac{owa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Optimizers  On Yago3-10 Based on the \ac{owa}
\begin{table*}[t]
\caption{Results Of Ablation Study For Optimizers On Yago3-10 Based on the \ac{owa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Optimizers  On NELL Based on the \ac{owa}
\begin{table*}[t]
\caption{Results Of Ablation Study For Optimizers On NELL Based on the \ac{owa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

\subsection{Study: Ablation Study For Optimizer Based On the \ac{lcwa}}

In our next ablation study, we investigated the effect of the optimizer when trained based on the \ac{lcwa}.
Again, we focused on ADADELTA~\cite{zeiler2012adadelta} and Adam~\cite{kingma2014adam}. 

% Results Of Ablation Study For Optimizers  On FB15k-237 Based On LCWA
\begin{table*}[t]
\caption{Results Of Ablation Study For Loss Functions On FB15k-237 Based On the \ac{lcwa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Optimizers  On WN18RR Based On LCWA
\begin{table*}[t]
\caption{Results Of Ablation Study For Loss Functions On WN18RR Based On LCWA.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Optimizers  On Yago3-10 Based On LCWA
\begin{table*}[t]
\caption{Results Of Ablation Study For Loss Functions On Yago3-10 Based On LCWA.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Loss Functions On NELL Based On LCWA
\begin{table*}[t]
\caption{Results Of Ablation Study For Optimizers  On NELL Based On LCWA.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

\subsection{Study: Ablation Study For Inverse Relations Based on the \ac{owa}}\label{ablation_inverse_relations_owa}

To investigate the effect of adding inverse relations to the \ac{kg}when trained based on the \ac{owa}, we performed a corresponding ablation study.
For each model, a \ac{hpo} was performed for both settings. 

% Results Of Ablation Study For Adding Inverse Relations To FB15k-237 Based on the \ac{owa}
\begin{table*}[t]
\caption{Results Of Ablation Study For Adding Inverse Relations To FB15k-237 Based on the \ac{owa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Optimizers  On WN18RR Based on the \ac{owa}
\begin{table*}[t]
\caption{Results Of Ablation Study For Adding Inverse Relations To WN18RR Based on the \ac{owa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Adding Inverse Relations To Yago3-10 Based on the \ac{owa}
\begin{table*}[t]
\caption{Results Of Ablation Study For Adding Inverse Relations To Yago3-10 Based on the \ac{owa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Adding Inverse Relations To NELL Based on the \ac{owa}
\begin{table*}[t]
\caption{Results Of Ablation Study For Adding Inverse Relations To NELL Based on the \ac{owa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

\subsection{Study: Ablation Study For Inverse Relations Based On the \ac{lcwa}}

Similar to \ref{ablation_inverse_relations_owa}, we investigated effect of adding inverse relations to the \ac{kg}on the model's performance.
The difference is that the models were trained based on the \ac{lcwa}.

% Results Of Ablation Study For Adding Inverse Relations To FB15k-237 Based On LCWA
\begin{table*}[t]
\caption{Results Of Ablation Study For Adding Inverse Relations To FB15k-237 Based On the \ac{lcwa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Adding Inverse Relations To WN18RR Based On LCWA
\begin{table*}[t]
\caption{Results Of Ablation Study For Adding Inverse Relations To WN18RR Based On the \ac{lcwa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Adding Inverse Relations To Yago3-10 Based On LCWA
\begin{table*}[t]
\caption{Results Of Ablation Study For Adding Inverse Relations To Yago3-10 Based On the \ac{lcwa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

% Results Of Ablation Study For Adding Inverse Relations To NELL Based On LCWA
\begin{table*}[t]
\caption{Results Of Ablation Study For Adding Inverse Relations To NELL Based On the \ac{lcwa}.}
\centering
\begin{tabular}{|llll|l|l|l|l|}
\hline
 &  &  &  & \multicolumn{4}{c|}{Hits@k} \\ \hline
\multicolumn{1}{|l|}{Model} & \multicolumn{1}{l|}{MR} & \multicolumn{1}{l|}{AMR} & MRR & Hits@1 & Hits@3 & Hits@5 & Hits@10 \\ \hline
\multicolumn{1}{|l|}{ComplEx~\cite{Trouillon2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvE~\cite{Dettmers2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ConvKB~\cite{nguyen2017novel}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{DistMult~\cite{Yang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ER-MLP~\cite{Dong2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{HolE~\cite{Nickel2016}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{KG2E~\cite{he2015learning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{NTN~\cite{socher2013reasoning}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{ProjE~\cite{shi2017proje}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RESCAL~\cite{Nickel2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{R-GCN~\cite{Schlichtkrull2018}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{RotatE~\cite{Sun2019}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SE~\cite{Bordes2011}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{SimplE~\cite{kazemi2018simple}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TuckER~\cite{balavzevic2019tucker}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransD~\cite{Ji2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransE~\cite{Bordes2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransH~\cite{Wang2014}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{TransR~\cite{Lin2015}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\multicolumn{1}{|l|}{UM~\cite{Glorot2013}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  &  &  &  \\ \hline
\end{tabular}%
\end{table*}

==> tables/relation_patterns_frequency.tex <==
\begin{tabular}{lrrr}
\toprule
pattern &  anti-symmetry &  composition &  symmetry \\
dataset  &                &              &           \\
\midrule
fb15k237 &            205 &          147 &         3 \\
wn18rr   &              7 &            1 &         3 \\
yago310  &             30 &            3 &         2 \\
\bottomrule
\end{tabular}

==> tables/reproducibility/fb15k237_table.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
       &   &      MRR (\%) &   Hits@1 (\%) &   Hits@3 (\%) &   Hits@5 (\%) &  Hits@10 (\%) &               MR &      AMR (\%) \\
\textbf{model} & {} &               &               &               &               &               &                  &               \\
\midrule
\textbf{\textcolor{NavyBlue}{ConvE}} & \textbf{pub (ND)} &     32.50 \phantom{$\pm$} \phantom{0.00} &     23.70 \phantom{$\pm$} \phantom{0.00} &     35.60 \phantom{$\pm$} \phantom{0.00} &               &     50.10 \phantom{$\pm$} \phantom{0.00} &     $\phantom{5}$244.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  29.69 $\pm$ 0.19 &  21.13 $\pm$ 0.21 &  32.32 $\pm$ 0.19 &  38.57 $\pm$ 0.12 &  47.19 $\pm$ 0.08 &  $\phantom{5}$245.83 $\pm$ $\phantom{5}$4.97 &  $\phantom{5}$3.45 $\pm$ 0.07 \\
\textbf{\textcolor{RedOrange}{ConvKB}} & \textbf{pub (O)} &     39.60 \phantom{$\pm$} \phantom{0.00} &               &               &               &     51.70 \phantom{$\pm$} \phantom{0.00} &     $\phantom{5}$257.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  $\phantom{5}$4.22 $\pm$ 0.18 &  $\phantom{5}$2.75 $\pm$ 0.27 &  $\phantom{5}$3.65 $\pm$ 0.19 &  $\phantom{5}$4.44 $\pm$ 0.19 &  $\phantom{5}$7.18 $\pm$ 0.71 &  4314.45 $\pm$ 27.24 &  60.46 $\pm$ 0.38 \\
\textbf{\textcolor{RedOrange}{MuRE}} & \textbf{pub (R)} &     33.60 \phantom{$\pm$} \phantom{0.00} &     24.50 \phantom{$\pm$} \phantom{0.00} &     37.00 \phantom{$\pm$} \phantom{0.00} &               &     52.10 \phantom{$\pm$} \phantom{0.00} &                  &               \\
       & \textbf{R} &  25.16 $\pm$ 0.20 &  16.12 $\pm$ 0.30 &  27.67 $\pm$ 0.21 &  34.21 $\pm$ 0.32 &  43.78 $\pm$ 0.13 &  $\phantom{5}$190.61 $\pm$ $\phantom{5}$0.58 &  $\phantom{5}$2.67 $\pm$ 0.01 \\
\textbf{\textcolor{RedOrange}{QuatE$^{1}$}} & \textbf{pub (O)} &     31.10 \phantom{$\pm$} \phantom{0.00} &     22.10 \phantom{$\pm$} \phantom{0.00} &     34.20 \phantom{$\pm$} \phantom{0.00} &               &     49.50 \phantom{$\pm$} \phantom{0.00} &     $\phantom{5}$176.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  $\phantom{5}$0.26 $\pm$ 0.02 &  $\phantom{5}$0.18 $\pm$ 0.03 &  $\phantom{5}$0.23 $\pm$ 0.02 &  $\phantom{5}$0.25 $\pm$ 0.02 &  $\phantom{5}$0.30 $\pm$ 0.01 &  7119.76 $\pm$ 36.06 &  99.78 $\pm$ 0.51 \\
\textbf{\textcolor{RedOrange}{RotatE}} & \textbf{pub (ND)} &     33.80 \phantom{$\pm$} \phantom{0.00} &     24.10 \phantom{$\pm$} \phantom{0.00} &     37.50 \phantom{$\pm$} \phantom{0.00} &               &     53.30 \phantom{$\pm$} \phantom{0.00} &     $\phantom{5}$177.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  28.79 $\pm$ 0.07 &  19.74 $\pm$ 0.08 &  31.67 $\pm$ 0.05 &  37.89 $\pm$ 0.07 &  47.13 $\pm$ 0.07 &  $\phantom{5}$176.70 $\pm$ $\phantom{5}$0.48 &  $\phantom{5}$2.48 $\pm$ 0.01 \\
\textbf{TuckER} & \textbf{pub (ND)} &     35.80 \phantom{$\pm$} \phantom{0.00} &     26.60 \phantom{$\pm$} \phantom{0.00} &     39.40 \phantom{$\pm$} \phantom{0.00} &               &     54.40 \phantom{$\pm$} \phantom{0.00} &                  &               \\
       & \textbf{R} &  35.51 $\pm$ 0.08 &  26.20 $\pm$ 0.15 &  39.05 $\pm$ 0.10 &  45.59 $\pm$ 0.12 &  54.11 $\pm$ 0.04 &  $\phantom{5}$152.46 $\pm$ $\phantom{5}$2.32 &  $\phantom{5}$2.14 $\pm$ 0.03 \\
\bottomrule
\end{tabular}



==> tables/reproducibility/fb15k237_table_without_std.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
       &   &           MRR (\%) &        Hits@1 (\%) &        Hits@3 (\%) &        Hits@5 (\%) &       Hits@10 (\%) &                             MR &           AMR (\%) \\
\textbf{Model} & {} &                    &                    &                    &                    &                    &                                &                    \\
\midrule
\textbf{\textcolor{NavyBlue}{ConvE}} & \textbf{pub} &  $32.5\phantom{0}$ &  $23.7\phantom{0}$ &  $35.6\phantom{0}$ &                    &  $50.1\phantom{0}$ &  $\phantom{0}244.\phantom{00}$ &                    \\
       & \textbf{R} &            $26.93$ &            $18.22$ &            $29.51$ &            $35.98$ &            $44.95$ &            $\phantom{0}255.46$ &  $\phantom{0}3.73$ \\\midrule
\textbf{\textcolor{RedOrange}{ConvKB}} & \textbf{pub} &  $39.6\phantom{0}$ &                    &                    &                    &  $51.7\phantom{0}$ &  $\phantom{0}257.\phantom{00}$ &                    \\
       & \textbf{R} &  $\phantom{0}4.71$ &  $\phantom{0}3.31$ &  $\phantom{0}4.04$ &  $\phantom{0}4.57$ &  $\phantom{0}7.76$ &                      $4345.27$ &            $61.36$ \\\midrule
\textbf{RotatE} & \textbf{pub} &  $33.8\phantom{0}$ &  $24.1\phantom{0}$ &  $37.5\phantom{0}$ &                    &  $53.3\phantom{0}$ &  $\phantom{0}177.\phantom{00}$ &                    \\
       & \textbf{R} &            $26.42$ &            $17.57$ &            $28.97$ &            $35.29$ &            $44.55$ &            $\phantom{0}191.92$ &  $\phantom{0}2.84$ \\
\bottomrule
\end{tabular}



==> tables/reproducibility/fb15k_table.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
       &   &       MRR (\%) &   Hits@1 (\%) &    Hits@3 (\%) &    Hits@5 (\%) &   Hits@10 (\%) &                MR &      AMR (\%) \\
\textbf{model} & {} &                &               &                &                &                &                   &               \\
\midrule
\textbf{\textcolor{RedOrange}{ComplEx}} & \textbf{pub (O)} &     69.20 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     59.90 \phantom{$\pm$} \phantom{0.00} &     75.90 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                &     84.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                   &               \\
       & \textbf{R} &  21.94 $\pm$ $\phantom{5}$0.71 &  12.73 $\pm$ 0.74 &  24.18 $\pm$ $\phantom{5}$0.65 &  30.67 $\pm$ $\phantom{5}$0.60 &  40.61 $\pm$ $\phantom{5}$0.74 &  $\phantom{5}$$\phantom{5}$170.56 $\pm$ 17.18 &  $\phantom{5}$2.31 $\pm$ 0.23 \\
\textbf{ConvE} & \textbf{pub (ND)} &     65.70 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     55.80 \phantom{$\pm$} \phantom{0.00} &     72.30 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                &     83.10 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$$\phantom{5}$51.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  75.45 $\pm$ $\phantom{5}$0.17 &  68.26 $\pm$ 0.27 &  80.47 $\pm$ $\phantom{5}$0.08 &  83.94 $\pm$ $\phantom{5}$0.01 &  87.68 $\pm$ $\phantom{5}$0.04 &  $\phantom{5}$$\phantom{5}$$\phantom{5}$43.97 $\pm$ $\phantom{5}$0.60 &  $\phantom{5}$0.60 $\pm$ 0.01 \\
\textbf{\textcolor{RedOrange}{DistMult}} & \textbf{pub (U)} &     35.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               &                &                &     57.70 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                   &               \\
       & \textbf{R} &  28.47 $\pm$ $\phantom{5}$0.23 &  18.59 $\pm$ 0.19 &  31.77 $\pm$ $\phantom{5}$0.29 &  38.24 $\pm$ $\phantom{5}$0.38 &  47.81 $\pm$ $\phantom{5}$0.36 &  $\phantom{5}$$\phantom{5}$127.16 $\pm$ $\phantom{5}$0.85 &  $\phantom{5}$1.72 $\pm$ 0.01 \\
\textbf{\textcolor{RedOrange}{HolE}} & \textbf{pub (ND)} &     52.40 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     40.20 \phantom{$\pm$} \phantom{0.00} &     61.30 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                &     73.90 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                   &               \\
       & \textbf{R} &  39.72 $\pm$ $\phantom{5}$0.32 &  27.15 $\pm$ 0.33 &  46.13 $\pm$ $\phantom{5}$0.40 &  54.05 $\pm$ $\phantom{5}$0.36 &  64.02 $\pm$ $\phantom{5}$0.27 &  $\phantom{5}$$\phantom{5}$186.22 $\pm$ $\phantom{5}$6.21 &  $\phantom{5}$2.52 $\pm$ 0.08 \\
\textbf{\textcolor{RedOrange}{KG2E}} & \textbf{pub (U)} &                &               &                &                &     71.50 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$$\phantom{5}$59.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  $\phantom{5}$0.63 $\pm$ $\phantom{5}$0.08 &  $\phantom{5}$0.15 $\pm$ 0.04 &  $\phantom{5}$0.41 $\pm$ $\phantom{5}$0.11 &  $\phantom{5}$0.66 $\pm$ $\phantom{5}$0.17 &  $\phantom{5}$1.25 $\pm$ $\phantom{5}$0.21 &  $\phantom{5}$5784.42 $\pm$ 22.26 &  78.31 $\pm$ 0.30 \\
\textbf{\textcolor{RedOrange}{QuatE$^{1}$}} & \textbf{pub (O)} &     77.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     70.00 \phantom{$\pm$} \phantom{0.00} &     82.10 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                &     87.80 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$$\phantom{5}$41.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  22.19 $\pm$ $\phantom{5}$0.17 &  14.65 $\pm$ 0.16 &  23.76 $\pm$ $\phantom{5}$0.26 &  29.37 $\pm$ $\phantom{5}$0.40 &  37.42 $\pm$ $\phantom{5}$0.39 &  $\phantom{5}$$\phantom{5}$229.99 $\pm$ $\phantom{5}$1.57 &  $\phantom{5}$3.11 $\pm$ 0.02 \\
\textbf{\textcolor{NavyBlue}{RotatE}} & \textbf{pub (ND)} &     79.70 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     74.60 \phantom{$\pm$} \phantom{0.00} &     83.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                &     88.40 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$$\phantom{5}$40.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  64.94 $\pm$ $\phantom{5}$0.03 &  53.05 $\pm$ 0.05 &  73.31 $\pm$ $\phantom{5}$0.06 &  78.74 $\pm$ $\phantom{5}$0.06 &  84.85 $\pm$ $\phantom{5}$0.03 &  $\phantom{5}$$\phantom{5}$$\phantom{5}$35.66 $\pm$ $\phantom{5}$0.06 &  $\phantom{5}$0.48 $\pm$ 0.00 \\
\textbf{\textcolor{RedOrange}{SimplE}} & \textbf{pub (O)} &     72.70 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     66.00 \phantom{$\pm$} \phantom{0.00} &     77.30 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                &     83.80 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                   &               \\
       & \textbf{R} &  $\phantom{5}$0.04 $\pm$ $\phantom{5}$0.00 &  $\phantom{5}$0.01 $\pm$ 0.00 &  $\phantom{5}$0.03 $\pm$ $\phantom{5}$0.01 &  $\phantom{5}$0.03 $\pm$ $\phantom{5}$0.01 &  $\phantom{5}$0.05 $\pm$ $\phantom{5}$0.00 &  $\phantom{5}$7386.02 $\pm$ $\phantom{5}$2.11 &  99.99 $\pm$ 0.03 \\
       & \textbf{O} &  23.62 $\pm$ 12.90 &  11.67 $\pm$ 8.68 &  24.65 $\pm$ 16.33 &  34.28 $\pm$ 20.19 &  51.91 $\pm$ 24.57 &  $\phantom{5}$$\phantom{5}$148.27 $\pm$ 89.28 &               \\
       & \textbf{P} &  $\phantom{5}$0.03 $\pm$ $\phantom{5}$0.00 &  $\phantom{5}$0.01 $\pm$ 0.00 &  $\phantom{5}$0.03 $\pm$ $\phantom{5}$0.01 &  $\phantom{5}$0.03 $\pm$ $\phantom{5}$0.01 &  $\phantom{5}$0.05 $\pm$ $\phantom{5}$0.00 &  14623.77 $\pm$ 91.95 &               \\
\textbf{\textcolor{RedOrange}{TransD}} & \textbf{pub (U)} &                &               &                &                &     77.30 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$$\phantom{5}$91.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  37.30 $\pm$ $\phantom{5}$0.05 &  24.45 $\pm$ 0.08 &  44.22 $\pm$ $\phantom{5}$0.09 &  51.78 $\pm$ $\phantom{5}$0.09 &  61.31 $\pm$ $\phantom{5}$0.07 &  $\phantom{5}$$\phantom{5}$146.55 $\pm$ $\phantom{5}$3.10 &  $\phantom{5}$1.98 $\pm$ 0.04 \\
\textbf{TransE} & \textbf{pub (U)} &                &               &                &                &     47.10 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$125.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  29.11 $\pm$ $\phantom{5}$0.20 &  17.99 $\pm$ 0.27 &  33.53 $\pm$ $\phantom{5}$0.18 &  40.76 $\pm$ $\phantom{5}$0.21 &  50.84 $\pm$ $\phantom{5}$0.28 &  $\phantom{5}$$\phantom{5}$122.01 $\pm$ $\phantom{5}$1.09 &  $\phantom{5}$1.65 $\pm$ 0.01 \\
\textbf{\textcolor{RedOrange}{TransH}} & \textbf{pub (U)} &                &               &                &                &     64.40 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$$\phantom{5}$87.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  $\phantom{5}$2.59 $\pm$ $\phantom{5}$0.27 &  $\phantom{5}$1.89 $\pm$ 0.35 &  $\phantom{5}$2.87 $\pm$ $\phantom{5}$0.23 &  $\phantom{5}$3.16 $\pm$ $\phantom{5}$0.11 &  $\phantom{5}$3.46 $\pm$ $\phantom{5}$0.15 &  $\phantom{5}$6318.90 $\pm$ 18.86 &  85.54 $\pm$ 0.26 \\
\textbf{\textcolor{RedOrange}{TransR}} & \textbf{pub (ND)} &                &               &                &                &     68.70 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$$\phantom{5}$77.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  $\phantom{5}$1.23 $\pm$ $\phantom{5}$0.04 &  $\phantom{5}$0.38 $\pm$ 0.00 &  $\phantom{5}$1.34 $\pm$ $\phantom{5}$0.10 &  $\phantom{5}$1.93 $\pm$ $\phantom{5}$0.12 &  $\phantom{5}$2.79 $\pm$ $\phantom{5}$0.09 &  $\phantom{5}$6130.41 $\pm$ $\phantom{5}$9.59 &  82.99 $\pm$ 0.13 \\
\textbf{TuckER} & \textbf{pub (ND)} &     79.50 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     74.10 \phantom{$\pm$} \phantom{0.00} &     83.30 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                &     89.20 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                   &               \\
       & \textbf{R} &  79.02 $\pm$ $\phantom{5}$0.12 &  73.10 $\pm$ 0.11 &  83.05 $\pm$ $\phantom{5}$0.13 &  85.93 $\pm$ $\phantom{5}$0.16 &  89.10 $\pm$ $\phantom{5}$0.10 &  $\phantom{5}$$\phantom{5}$$\phantom{5}$40.35 $\pm$ $\phantom{5}$0.83 &  $\phantom{5}$0.55 $\pm$ 0.01 \\
\bottomrule
\label{tab:fb15k_table_without_std}
\end{tabular}



==> tables/reproducibility/fb15k_table_without_std.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
       &   &           MRR (\%) &        Hits@1 (\%) &        Hits@3 (\%) &        Hits@5 (\%) &       Hits@10 (\%) &                              MR &            AMR (\%) \\
\textbf{Model} & {} &                    &                    &                    &                    &                    &                                 &                     \\
\midrule
\textbf{ComplEx} & \textbf{pub} &  $69.2\phantom{0}$ &  $59.9\phantom{0}$ &  $75.9\phantom{0}$ &                    &  $84.\phantom{00}$ &                                 &                     \\
       & \textbf{R} &            $19.13$ &            $10.06$ &            $20.82$ &            $27.59$ &            $38.03$ &            $\phantom{00}171.16$ &  $\phantom{00}2.46$ \\\midrule
\textbf{\textcolor{NavyBlue}{ConvE}} & \textbf{pub} &  $65.7\phantom{0}$ &  $55.8\phantom{0}$ &  $72.3\phantom{0}$ &                    &  $83.1\phantom{0}$ &  $\phantom{000}51.\phantom{00}$ &                     \\
       & \textbf{R} &            $59.56$ &            $48.28$ &            $66.99$ &            $73.27$ &            $79.76$ &            $\phantom{000}50.76$ &  $\phantom{00}0.73$ \\\midrule
\textbf{DistMult} & \textbf{pub} &  $35.\phantom{00}$ &                    &                    &                    &  $57.7\phantom{0}$ &                                 &                     \\
       & \textbf{R} &            $26.06$ &            $16.45$ &            $29.10$ &            $35.54$ &            $45.00$ &            $\phantom{00}134.02$ &  $\phantom{00}1.86$ \\\midrule
\textbf{HolE} & \textbf{pub} &  $52.4\phantom{0}$ &  $40.2\phantom{0}$ &  $61.3\phantom{0}$ &                    &  $73.9\phantom{0}$ &                                 &                     \\
       & \textbf{R} &            $34.15$ &            $21.79$ &            $39.69$ &            $48.06$ &            $58.84$ &            $\phantom{00}193.03$ &  $\phantom{00}2.71$ \\\midrule
\textbf{\textcolor{RedOrange}{KG2E}} & \textbf{pub} &                    &                    &                    &                    &  $71.5\phantom{0}$ &  $\phantom{000}59.\phantom{00}$ &                     \\
       & \textbf{R} &  $\phantom{0}0.58$ &  $\phantom{0}0.11$ &  $\phantom{0}0.36$ &  $\phantom{0}0.56$ &  $\phantom{0}1.01$ &            $\phantom{0}5779.07$ &  $\phantom{0}78.40$ \\\midrule
\textbf{RotatE} & \textbf{pub} &  $79.7\phantom{0}$ &  $74.6\phantom{0}$ &  $83.\phantom{00}$ &                    &  $88.4\phantom{0}$ &  $\phantom{000}40.\phantom{00}$ &                     \\
       & \textbf{R} &            $55.00$ &            $41.53$ &            $64.14$ &            $71.23$ &            $78.67$ &            $\phantom{000}42.28$ &  $\phantom{00}0.63$ \\\midrule
\textbf{\textcolor{RedOrange}{SimplE}} & \textbf{pub} &  $72.7\phantom{0}$ &  $66.\phantom{00}$ &  $77.3\phantom{0}$ &                    &  $83.8\phantom{0}$ &                                 &                     \\
       & \textbf{R} &  $\phantom{0}0.04$ &  $\phantom{0}0.01$ &  $\phantom{0}0.03$ &  $\phantom{0}0.04$ &  $\phantom{0}0.06$ &            $\phantom{0}7395.75$ &            $100.02$ \\
       & \textbf{O} &            $23.90$ &            $11.58$ &            $24.16$ &            $34.73$ &            $54.28$ &            $\phantom{00}139.34$ &                     \\
       & \textbf{P} &  $\phantom{0}0.03$ &  $\phantom{0}0.01$ &  $\phantom{0}0.03$ &  $\phantom{0}0.04$ &  $\phantom{0}0.06$ &                      $14652.16$ &                     \\\midrule
\textbf{TransD} & \textbf{pub} &                    &                    &                    &                    &  $77.3\phantom{0}$ &  $\phantom{000}91.\phantom{00}$ &                     \\
       & \textbf{R} &            $33.99$ &            $21.22$ &            $40.48$ &            $48.57$ &            $58.71$ &            $\phantom{00}153.37$ &  $\phantom{00}2.29$ \\\midrule
\textbf{\textcolor{NavyBlue}{TransE}} & \textbf{pub} &                    &                    &                    &                    &  $47.1\phantom{0}$ &  $\phantom{00}125.\phantom{00}$ &                     \\
       & \textbf{R} &            $26.01$ &            $15.23$ &            $29.85$ &            $37.18$ &            $47.34$ &            $\phantom{00}127.92$ &  $\phantom{00}1.78$ \\\midrule
\textbf{\textcolor{RedOrange}{TransH}} & \textbf{pub} &                    &                    &                    &                    &  $64.4\phantom{0}$ &  $\phantom{000}87.\phantom{00}$ &                     \\
       & \textbf{R} &  $\phantom{0}2.54$ &  $\phantom{0}1.69$ &  $\phantom{0}2.95$ &  $\phantom{0}3.29$ &  $\phantom{0}3.74$ &            $\phantom{0}6320.02$ &  $\phantom{0}85.63$ \\
       & \textbf{O} &  $\phantom{0}2.54$ &  $\phantom{0}1.69$ &  $\phantom{0}2.95$ &  $\phantom{0}3.29$ &  $\phantom{0}3.74$ &            $\phantom{0}6320.00$ &                     \\
       & \textbf{P} &  $\phantom{0}2.54$ &  $\phantom{0}1.69$ &  $\phantom{0}2.95$ &  $\phantom{0}3.29$ &  $\phantom{0}3.74$ &            $\phantom{0}6320.05$ &                     \\\midrule
\textbf{\textcolor{RedOrange}{TransR}} & \textbf{pub} &                    &                    &                    &                    &  $68.7\phantom{0}$ &  $\phantom{000}77.\phantom{00}$ &                     \\
       & \textbf{R} &  $\phantom{0}0.65$ &  $\phantom{0}0.37$ &  $\phantom{0}0.63$ &  $\phantom{0}0.78$ &  $\phantom{0}1.03$ &            $\phantom{0}6795.95$ &  $\phantom{0}91.99$ \\
       & \textbf{O} &  $\phantom{0}0.65$ &  $\phantom{0}0.37$ &  $\phantom{0}0.63$ &  $\phantom{0}0.78$ &  $\phantom{0}1.03$ &            $\phantom{0}6795.94$ &                     \\
       & \textbf{P} &  $\phantom{0}0.65$ &  $\phantom{0}0.37$ &  $\phantom{0}0.63$ &  $\phantom{0}0.78$ &  $\phantom{0}1.03$ &            $\phantom{0}6795.95$ &                     \\\midrule
\textbf{\textcolor{RedOrange}{TuckER}} & \textbf{pub} &  $79.5\phantom{0}$ &  $74.1\phantom{0}$ &  $83.3\phantom{0}$ &                    &  $89.2\phantom{0}$ &                                 &                     \\
       & \textbf{R} &  $\phantom{0}0.07$ &  $\phantom{0}0.01$ &  $\phantom{0}0.02$ &  $\phantom{0}0.03$ &  $\phantom{0}0.15$ &            $\phantom{0}7327.77$ &  $\phantom{0}99.11$ \\
\bottomrule
\end{tabular}



==> tables/reproducibility/wn18_table.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
       &   &      MRR (\%) &   Hits@1 (\%) &   Hits@3 (\%) &   Hits@5 (\%) &   Hits@10 (\%) &                 MR &      AMR (\%) \\
\textbf{model} & {} &               &               &               &               &                &                    &               \\
\midrule
\textbf{\textcolor{RedOrange}{ComplEx}} & \textbf{pub (O)} &     94.10 \phantom{$\pm$} \phantom{0.00} &     93.60 \phantom{$\pm$} \phantom{0.00} &     94.50 \phantom{$\pm$} \phantom{0.00} &               &     94.70 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                    &               \\
       & \textbf{R} &  18.28 $\pm$ 2.10 &  11.65 $\pm$ 1.32 &  19.04 $\pm$ 2.44 &  23.38 $\pm$ 3.06 &  30.70 $\pm$ $\phantom{5}$3.90 &  $\phantom{5}$$\phantom{5}$442.51 $\pm$ $\phantom{5}$47.32 &  $\phantom{5}$2.16 $\pm$ 0.23 \\
\textbf{ConvE} & \textbf{pub (ND)} &     94.30 \phantom{$\pm$} \phantom{0.00} &     93.50 \phantom{$\pm$} \phantom{0.00} &     94.60 \phantom{$\pm$} \phantom{0.00} &               &     95.60 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$374.00 \phantom{$\pm$} $\phantom{5}$$\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  94.23 $\pm$ 0.08 &  93.54 $\pm$ 0.16 &  94.68 $\pm$ 0.04 &  95.03 $\pm$ 0.02 &  95.39 $\pm$ $\phantom{5}$0.09 &  $\phantom{5}$$\phantom{5}$462.53 $\pm$ $\phantom{5}$32.15 &  $\phantom{5}$2.26 $\pm$ 0.16 \\
\textbf{DistMult} & \textbf{pub (U)} &     83.00 \phantom{$\pm$} \phantom{0.00} &               &               &               &     94.20 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                    &               \\
       & \textbf{R} &  82.41 $\pm$ 0.24 &  74.74 $\pm$ 0.31 &  89.09 $\pm$ 0.19 &  91.36 $\pm$ 0.22 &  93.44 $\pm$ $\phantom{5}$0.15 &  $\phantom{5}$$\phantom{5}$454.41 $\pm$ $\phantom{5}$43.08 &  $\phantom{5}$2.22 $\pm$ 0.21 \\
\textbf{\textcolor{RedOrange}{HolE}} & \textbf{pub (ND)} &     93.80 \phantom{$\pm$} \phantom{0.00} &     93.00 \phantom{$\pm$} \phantom{0.00} &     94.50 \phantom{$\pm$} \phantom{0.00} &               &     94.90 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                    &               \\
       & \textbf{R} &  73.43 $\pm$ 0.40 &  63.22 $\pm$ 0.57 &  81.80 $\pm$ 0.40 &  85.81 $\pm$ 0.20 &  89.30 $\pm$ $\phantom{5}$0.26 &  $\phantom{5}$$\phantom{5}$786.05 $\pm$ $\phantom{5}$33.16 &  $\phantom{5}$3.84 $\pm$ 0.16 \\
\textbf{\textcolor{RedOrange}{KG2E}} & \textbf{pub (U)} &               &               &               &               &     92.80 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$331.00 \phantom{$\pm$} $\phantom{5}$$\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  $\phantom{5}$3.73 $\pm$ 0.22 &  $\phantom{5}$1.46 $\pm$ 0.19 &  $\phantom{5}$3.27 $\pm$ 0.26 &  $\phantom{5}$4.77 $\pm$ 0.32 &  $\phantom{5}$7.39 $\pm$ $\phantom{5}$0.33 &  $\phantom{5}$2732.49 $\pm$ $\phantom{5}$57.69 &  13.35 $\pm$ 0.28 \\
       & \textbf{O} &  $\phantom{5}$3.74 $\pm$ 0.22 &  $\phantom{5}$1.46 $\pm$ 0.19 &  $\phantom{5}$3.27 $\pm$ 0.26 &  $\phantom{5}$4.77 $\pm$ 0.32 &  $\phantom{5}$7.39 $\pm$ $\phantom{5}$0.33 &  $\phantom{5}$2732.49 $\pm$ $\phantom{5}$57.69 &               \\
\textbf{\textcolor{RedOrange}{QuatE$^{1}$}} & \textbf{pub (O)} &     94.90 \phantom{$\pm$} \phantom{0.00} &     94.10 \phantom{$\pm$} \phantom{0.00} &     95.40 \phantom{$\pm$} \phantom{0.00} &               &     96.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$388.00 \phantom{$\pm$} $\phantom{5}$$\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  67.28 $\pm$ 0.70 &  58.38 $\pm$ 0.88 &  73.05 $\pm$ 0.61 &  77.86 $\pm$ 0.53 &  83.25 $\pm$ $\phantom{5}$0.38 &  $\phantom{5}$$\phantom{5}$327.12 $\pm$ $\phantom{5}$12.44 &  $\phantom{5}$1.60 $\pm$ 0.06 \\
\textbf{RotatE} & \textbf{pub (ND)} &     94.90 \phantom{$\pm$} \phantom{0.00} &     94.40 \phantom{$\pm$} \phantom{0.00} &     95.20 \phantom{$\pm$} \phantom{0.00} &               &     95.90 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$309.00 \phantom{$\pm$} $\phantom{5}$$\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  93.71 $\pm$ 0.03 &  92.27 $\pm$ 0.03 &  94.87 $\pm$ 0.06 &  95.34 $\pm$ 0.04 &  95.83 $\pm$ $\phantom{5}$0.05 &  $\phantom{5}$$\phantom{5}$270.22 $\pm$ $\phantom{5}$$\phantom{5}$7.24 &  $\phantom{5}$1.32 $\pm$ 0.04 \\
\textbf{\textcolor{RedOrange}{SimplE}} & \textbf{pub (O)} &     94.20 \phantom{$\pm$} \phantom{0.00} &     93.90 \phantom{$\pm$} \phantom{0.00} &     94.40 \phantom{$\pm$} \phantom{0.00} &               &     94.70 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                    &               \\
       & \textbf{R} &  $\phantom{5}$0.04 $\pm$ 0.02 &  $\phantom{5}$0.01 $\pm$ 0.01 &  $\phantom{5}$0.03 $\pm$ 0.02 &  $\phantom{5}$0.04 $\pm$ 0.03 &  $\phantom{5}$0.06 $\pm$ $\phantom{5}$0.03 &  20355.98 $\pm$ $\phantom{5}$19.42 &  99.48 $\pm$ 0.09 \\
       & \textbf{O} &  32.95 $\pm$ 8.10 &  28.19 $\pm$ 6.94 &  33.94 $\pm$ 8.84 &  37.28 $\pm$ 9.69 &  42.40 $\pm$ 10.53 &  $\phantom{5}$$\phantom{5}$469.49 $\pm$ 161.36 &               \\
       & \textbf{P} &  $\phantom{5}$0.03 $\pm$ 0.01 &  $\phantom{5}$0.01 $\pm$ 0.01 &  $\phantom{5}$0.03 $\pm$ 0.02 &  $\phantom{5}$0.04 $\pm$ 0.03 &  $\phantom{5}$0.06 $\pm$ $\phantom{5}$0.03 &  40242.47 $\pm$ 195.66 &               \\
\textbf{\textcolor{NavyBlue}{TransD}} & \textbf{pub (U)} &               &               &               &               &     92.20 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$212.00 \phantom{$\pm$} $\phantom{5}$$\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  37.33 $\pm$ 0.52 &  $\phantom{5}$4.31 $\pm$ 0.42 &  67.90 $\pm$ 0.93 &  81.01 $\pm$ 0.30 &  87.80 $\pm$ $\phantom{5}$0.33 &  $\phantom{5}$$\phantom{5}$460.00 $\pm$ $\phantom{5}$$\phantom{5}$7.40 &  $\phantom{5}$2.25 $\pm$ 0.04 \\
\textbf{\textcolor{RedOrange}{TransE}} & \textbf{pub (U)} &               &               &               &               &     89.20 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$251.00 \phantom{$\pm$} $\phantom{5}$$\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  37.04 $\pm$ 1.37 &  $\phantom{5}$9.29 $\pm$ 1.83 &  60.28 $\pm$ 1.25 &  72.02 $\pm$ 0.75 &  81.51 $\pm$ $\phantom{5}$0.52 &  $\phantom{5}$$\phantom{5}$489.84 $\pm$ $\phantom{5}$42.13 &  $\phantom{5}$2.39 $\pm$ 0.21 \\
\textbf{\textcolor{RedOrange}{TransH}} & \textbf{pub (U)} &               &               &               &               &     82.30 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$388.00 \phantom{$\pm$} $\phantom{5}$$\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  $\phantom{5}$0.17 $\pm$ 0.17 &  $\phantom{5}$0.08 $\pm$ 0.12 &  $\phantom{5}$0.17 $\pm$ 0.20 &  $\phantom{5}$0.21 $\pm$ 0.24 &  $\phantom{5}$0.31 $\pm$ $\phantom{5}$0.29 &  19551.68 $\pm$ 166.54 &  95.55 $\pm$ 0.81 \\
\textbf{\textcolor{RedOrange}{TransR}} & \textbf{pub (ND)} &               &               &               &               &     92.00 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &     $\phantom{5}$$\phantom{5}$225.00 \phantom{$\pm$} $\phantom{5}$$\phantom{5}$\phantom{0.00} &               \\
       & \textbf{R} &  $\phantom{5}$0.24 $\pm$ 0.03 &  $\phantom{5}$0.00 $\pm$ 0.01 &  $\phantom{5}$0.22 $\pm$ 0.05 &  $\phantom{5}$0.38 $\pm$ 0.05 &  $\phantom{5}$0.63 $\pm$ $\phantom{5}$0.07 &  18882.20 $\pm$ 240.51 &  92.27 $\pm$ 1.18 \\
\textbf{TuckER} & \textbf{pub (ND)} &     95.30 \phantom{$\pm$} \phantom{0.00} &     94.90 \phantom{$\pm$} \phantom{0.00} &     95.50 \phantom{$\pm$} \phantom{0.00} &               &     95.80 \phantom{$\pm$} $\phantom{5}$\phantom{0.00} &                    &               \\
       & \textbf{R} &  94.89 $\pm$ 0.05 &  94.52 $\pm$ 0.05 &  95.17 $\pm$ 0.07 &  95.30 $\pm$ 0.07 &  95.50 $\pm$ $\phantom{5}$0.06 &  $\phantom{5}$$\phantom{5}$532.05 $\pm$ $\phantom{5}$45.91 &  $\phantom{5}$2.60 $\pm$ 0.22 \\
\bottomrule
\end{tabular}




==> tables/reproducibility/wn18_table_without_std.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
       &   &           MRR (\%) &        Hits@1 (\%) &        Hits@3 (\%) &        Hits@5 (\%) &       Hits@10 (\%) &                              MR &            AMR (\%) \\
\textbf{Model} & {} &                    &                    &                    &                    &                    &                                 &                     \\
\midrule
\textbf{ComplEx} & \textbf{pub} &  $94.1\phantom{0}$ &  $93.6\phantom{0}$ &  $94.5\phantom{0}$ &                    &  $94.7\phantom{0}$ &                                 &                     \\
       & \textbf{R} &            $19.49$ &            $12.36$ &            $20.66$ &            $25.24$ &            $32.92$ &            $\phantom{00}452.67$ &  $\phantom{00}2.21$ \\\midrule
\textbf{\textcolor{NavyBlue}{ConvE}} & \textbf{pub} &  $94.3\phantom{0}$ &  $93.5\phantom{0}$ &  $94.6\phantom{0}$ &                    &  $95.6\phantom{0}$ &  $\phantom{00}374.\phantom{00}$ &                     \\
       & \textbf{R} &            $88.81$ &            $85.14$ &            $91.76$ &            $93.29$ &            $94.85$ &            $\phantom{00}444.40$ &  $\phantom{00}2.17$ \\\midrule
\textbf{\textcolor{NavyBlue}{DistMult}} & \textbf{pub} &  $83.\phantom{00}$ &                    &                    &                    &  $94.2\phantom{0}$ &                                 &                     \\
       & \textbf{R} &            $77.44$ &            $67.45$ &            $85.94$ &            $89.52$ &            $92.72$ &            $\phantom{00}458.64$ &  $\phantom{00}2.24$ \\\midrule
\textbf{\textcolor{NavyBlue}{HolE}} & \textbf{pub} &  $93.8\phantom{0}$ &  $93.\phantom{00}$ &  $94.5\phantom{0}$ &                    &  $94.9\phantom{0}$ &                                 &                     \\
       & \textbf{R} &            $70.44$ &            $59.29$ &            $79.29$ &            $84.12$ &            $88.61$ &            $\phantom{00}812.64$ &  $\phantom{00}3.97$ \\
       & \textbf{O} &            $70.44$ &            $59.29$ &            $79.29$ &            $84.12$ &            $88.61$ &            $\phantom{00}812.63$ &                     \\
       & \textbf{P} &            $70.44$ &            $59.29$ &            $79.29$ &            $84.12$ &            $88.61$ &            $\phantom{00}812.64$ &                     \\\midrule
\textbf{\textcolor{RedOrange}{KG2E}} & \textbf{pub} &                    &                    &                    &                    &  $92.8\phantom{0}$ &  $\phantom{00}331.\phantom{00}$ &                     \\
       & \textbf{R} &  $\phantom{0}3.61$ &  $\phantom{0}1.35$ &  $\phantom{0}3.21$ &  $\phantom{0}4.57$ &  $\phantom{0}7.02$ &            $\phantom{0}2708.89$ &  $\phantom{0}13.25$ \\
       & \textbf{O} &  $\phantom{0}3.61$ &  $\phantom{0}1.35$ &  $\phantom{0}3.21$ &  $\phantom{0}4.57$ &  $\phantom{0}7.02$ &            $\phantom{0}2708.88$ &                     \\
       & \textbf{P} &  $\phantom{0}3.61$ &  $\phantom{0}1.35$ &  $\phantom{0}3.21$ &  $\phantom{0}4.57$ &  $\phantom{0}7.02$ &            $\phantom{0}2708.89$ &                     \\\midrule
\textbf{\textcolor{NavyBlue}{RotatE}} & \textbf{pub} &  $94.9\phantom{0}$ &  $94.4\phantom{0}$ &  $95.2\phantom{0}$ &                    &  $95.9\phantom{0}$ &  $\phantom{00}309.\phantom{00}$ &                     \\
       & \textbf{R} &            $87.29$ &            $82.17$ &            $91.53$ &            $93.44$ &            $95.28$ &            $\phantom{00}123.68$ &  $\phantom{00}0.61$ \\\midrule
\textbf{\textcolor{RedOrange}{SimplE}} & \textbf{pub} &  $94.2\phantom{0}$ &  $93.9\phantom{0}$ &  $94.4\phantom{0}$ &                    &  $94.7\phantom{0}$ &                                 &                     \\
       & \textbf{R} &  $\phantom{0}0.04$ &  $\phantom{0}0.01$ &  $\phantom{0}0.03$ &  $\phantom{0}0.04$ &  $\phantom{0}0.07$ &                      $20376.43$ &  $\phantom{0}99.57$ \\
       & \textbf{O} &            $38.48$ &            $33.93$ &            $39.59$ &            $42.76$ &            $47.01$ &            $\phantom{00}384.53$ &                     \\
       & \textbf{P} &  $\phantom{0}0.03$ &  $\phantom{0}0.01$ &  $\phantom{0}0.03$ &  $\phantom{0}0.04$ &  $\phantom{0}0.07$ &                      $40368.33$ &                     \\\midrule
\textbf{\textcolor{NavyBlue}{TransD}} & \textbf{pub} &                    &                    &                    &                    &  $92.2\phantom{0}$ &  $\phantom{00}212.\phantom{00}$ &                     \\
       & \textbf{R} &            $36.22$ &  $\phantom{0}3.94$ &            $65.63$ &            $79.64$ &            $87.27$ &            $\phantom{00}444.39$ &  $\phantom{00}2.17$ \\\midrule
\textbf{\textcolor{NavyBlue}{TransE}} & \textbf{pub} &                    &                    &                    &                    &  $89.2\phantom{0}$ &  $\phantom{00}251.\phantom{00}$ &                     \\
       & \textbf{R} &            $39.19$ &  $\phantom{0}9.99$ &            $64.74$ &            $75.44$ &            $84.25$ &            $\phantom{00}468.24$ &  $\phantom{00}2.29$ \\\midrule
\textbf{\textcolor{RedOrange}{TransH}} & \textbf{pub} &                    &                    &                    &                    &  $82.3\phantom{0}$ &  $\phantom{00}388.\phantom{00}$ &                     \\
       & \textbf{R} &  $\phantom{0}0.18$ &  $\phantom{0}0.04$ &  $\phantom{0}0.19$ &  $\phantom{0}0.29$ &  $\phantom{0}0.39$ &                      $19678.04$ &  $\phantom{0}96.16$ \\
       & \textbf{O} &  $\phantom{0}0.18$ &  $\phantom{0}0.04$ &  $\phantom{0}0.19$ &  $\phantom{0}0.29$ &  $\phantom{0}0.39$ &                      $19678.02$ &                     \\
       & \textbf{P} &  $\phantom{0}0.18$ &  $\phantom{0}0.04$ &  $\phantom{0}0.19$ &  $\phantom{0}0.29$ &  $\phantom{0}0.39$ &                      $19678.06$ &                     \\\midrule
\textbf{\textcolor{RedOrange}{TransR}} & \textbf{pub} &                    &                    &                    &                    &  $92.\phantom{00}$ &  $\phantom{00}225.\phantom{00}$ &                     \\
       & \textbf{R} &  $\phantom{0}0.06$ &  $\phantom{0}0.00$ &  $\phantom{0}0.04$ &  $\phantom{0}0.05$ &  $\phantom{0}0.11$ &                      $19686.49$ &  $\phantom{0}96.20$ \\
       & \textbf{O} &  $\phantom{0}0.06$ &  $\phantom{0}0.00$ &  $\phantom{0}0.04$ &  $\phantom{0}0.05$ &  $\phantom{0}0.11$ &                      $19686.49$ &                     \\
       & \textbf{P} &  $\phantom{0}0.06$ &  $\phantom{0}0.00$ &  $\phantom{0}0.04$ &  $\phantom{0}0.05$ &  $\phantom{0}0.11$ &                      $19686.50$ &                     \\\midrule
\textbf{\textcolor{RedOrange}{TuckER}} & \textbf{pub} &  $95.3\phantom{0}$ &  $94.9\phantom{0}$ &  $95.5\phantom{0}$ &                    &  $95.8\phantom{0}$ &                                 &                     \\
       & \textbf{R} &  $\phantom{0}0.03$ &  $\phantom{0}0.00$ &  $\phantom{0}0.02$ &  $\phantom{0}0.03$ &  $\phantom{0}0.04$ &                      $20622.46$ &            $100.78$ \\
\bottomrule
\end{tabular}



==> tables/reproducibility/wn18rr_table.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
       &   &      MRR (\%) &   Hits@1 (\%) &   Hits@3 (\%) &   Hits@5 (\%) &  Hits@10 (\%) &                 MR &       AMR (\%) \\
\textbf{model} & {} &               &               &               &               &               &                    &                \\
\midrule
\textbf{ConvE} & \textbf{pub (ND)} &     43.00 \phantom{$\pm$} \phantom{0.00} &     40.00 \phantom{$\pm$} \phantom{0.00} &     44.00 \phantom{$\pm$} \phantom{0.00} &               &     52.00 \phantom{$\pm$} \phantom{0.00} &     $\phantom{5}$4187.00 \phantom{$\pm$} $\phantom{5}$$\phantom{5}$\phantom{0.00} &                \\
       & \textbf{R} &  45.28 $\pm$ 0.13 &  41.93 $\pm$ 0.19 &  46.64 $\pm$ 0.25 &  49.07 $\pm$ 0.22 &  51.98 $\pm$ 0.24 &  $\phantom{5}$5203.77 $\pm$ 129.07 &  $\phantom{5}$25.67 $\pm$ 0.64 \\
\textbf{\textcolor{RedOrange}{ConvKB}} & \textbf{pub (O)} &     24.80 \phantom{$\pm$} \phantom{0.00} &               &               &               &     52.50 \phantom{$\pm$} \phantom{0.00} &     $\phantom{5}$2554.00 \phantom{$\pm$} $\phantom{5}$$\phantom{5}$\phantom{0.00} &                \\
       & \textbf{R} &  $\phantom{5}$0.34 $\pm$ 0.05 &  $\phantom{5}$0.11 $\pm$ 0.04 &  $\phantom{5}$0.27 $\pm$ 0.02 &  $\phantom{5}$0.43 $\pm$ 0.06 &  $\phantom{5}$0.63 $\pm$ 0.08 &  13905.99 $\pm$ 962.71 &  $\phantom{5}$68.60 $\pm$ 4.75 \\
\textbf{\textcolor{RedOrange}{QuatE$^{1}$}} & \textbf{pub (O)} &     48.10 \phantom{$\pm$} \phantom{0.00} &     43.60 \phantom{$\pm$} \phantom{0.00} &     50.00 \phantom{$\pm$} \phantom{0.00} &               &     56.40 \phantom{$\pm$} \phantom{0.00} &     $\phantom{5}$3472.00 \phantom{$\pm$} $\phantom{5}$$\phantom{5}$\phantom{0.00} &                \\
       & \textbf{R} &  $\phantom{5}$0.58 $\pm$ 0.05 &  $\phantom{5}$0.38 $\pm$ 0.06 &  $\phantom{5}$0.56 $\pm$ 0.08 &  $\phantom{5}$0.66 $\pm$ 0.06 &  $\phantom{5}$0.88 $\pm$ 0.09 &  20404.47 $\pm$ 196.81 &  100.65 $\pm$ 0.97 \\
\textbf{RotatE} & \textbf{pub (ND)} &     47.60 \phantom{$\pm$} \phantom{0.00} &     42.80 \phantom{$\pm$} \phantom{0.00} &     49.20 \phantom{$\pm$} \phantom{0.00} &               &     57.10 \phantom{$\pm$} \phantom{0.00} &     $\phantom{5}$3340.00 \phantom{$\pm$} $\phantom{5}$$\phantom{5}$\phantom{0.00} &                \\
       & \textbf{R} &  49.39 $\pm$ 0.06 &  45.49 $\pm$ 0.12 &  51.03 $\pm$ 0.10 &  53.36 $\pm$ 0.15 &  57.05 $\pm$ 0.14 &  $\phantom{5}$4046.79 $\pm$ $\phantom{5}$89.15 &  $\phantom{5}$19.96 $\pm$ 0.44 \\
\textbf{TuckER} & \textbf{pub (ND)} &     47.00 \phantom{$\pm$} \phantom{0.00} &     44.30 \phantom{$\pm$} \phantom{0.00} &     48.20 \phantom{$\pm$} \phantom{0.00} &               &     52.60 \phantom{$\pm$} \phantom{0.00} &                    &                \\
       & \textbf{R} &  47.62 $\pm$ 0.58 &  44.91 $\pm$ 0.62 &  48.81 $\pm$ 0.59 &  50.40 $\pm$ 0.58 &  52.80 $\pm$ 0.45 &  $\phantom{5}$5646.84 $\pm$ 146.30 &  $\phantom{5}$27.85 $\pm$ 0.72 \\
\bottomrule
\label{tab:wn18rr_table_without_std}
\end{tabular}



==> tables/reproducibility/wn18rr_table_without_std.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
       &   &           MRR (\%) &                  Hits@1 (\%) &        Hits@3 (\%) &        Hits@5 (\%) &       Hits@10 (\%) &                              MR & AMR (\%) \\
\textbf{Model} & {} &                    &                              &                    &                    &                    &                                 &          \\
\midrule
\textbf{\textcolor{NavyBlue}{ConvE}} & \textbf{pub} &  $43.\phantom{00}$ &  $\phantom{0}4.\phantom{00}$ &  $44.\phantom{00}$ &                    &  $52.\phantom{00}$ &  $\phantom{0}4187.\phantom{00}$ &          \\
       & \textbf{R} &            $44.69$ &                      $40.98$ &            $46.49$ &            $48.92$ &            $51.76$ &            $\phantom{0}5369.49$ &  $26.49$ \\\midrule
\textbf{\textcolor{RedOrange}{ConvKB}} & \textbf{pub} &  $24.8\phantom{0}$ &                              &                    &                    &  $52.5\phantom{0}$ &  $\phantom{0}2554.\phantom{00}$ &          \\
       & \textbf{R} &  $\phantom{0}0.30$ &            $\phantom{0}0.09$ &  $\phantom{0}0.21$ &  $\phantom{0}0.32$ &  $\phantom{0}0.57$ &                      $13634.66$ &  $67.27$ \\
       & \textbf{O} &  $\phantom{0}0.30$ &            $\phantom{0}0.09$ &  $\phantom{0}0.21$ &  $\phantom{0}0.32$ &  $\phantom{0}0.57$ &                      $13634.65$ &          \\
       & \textbf{P} &  $\phantom{0}0.30$ &            $\phantom{0}0.09$ &  $\phantom{0}0.21$ &  $\phantom{0}0.32$ &  $\phantom{0}0.57$ &                      $13634.66$ &          \\\midrule
\textbf{\textcolor{NavyBlue}{RotatE}} & \textbf{pub} &  $47.6\phantom{0}$ &            $42.8\phantom{0}$ &  $49.2\phantom{0}$ &                    &  $57.1\phantom{0}$ &  $\phantom{0}3340.\phantom{00}$ &          \\
       & \textbf{R} &            $48.40$ &                      $44.02$ &            $50.55$ &            $52.98$ &            $56.51$ &            $\phantom{0}4263.32$ &  $21.03$ \\
\bottomrule
\end{tabular}



==> tables/reproduction.tex <==
%
%
%
%
%
%
%

%
%
%
%
%
%

%
%
%
%
%
%

%
%
%
%
%
%


\begin{table}[H]
    \centering
    \caption{Reproduction of Studies on FB15K where \textbf{pub} refers to published results, \textbf{R} to results based on the realistic ranking, \textbf{O} to results based on the optimistic ranking, and \textbf{P} to results based on the pessimistic ranking. 
    For published results, there are two additional rank types, \textbf{U} for undefined due to missing official implementation and \textbf{ND} for non-deterministic.
    We only show the results of the optimistic and pessimistic ranking in case they differ from the realistic ranking.}
    \label{tab:rps_fb15k}
    \input{tables/reproducibility/fb15k_table}
\end{table}


\begin{table}[H]
    \centering
    \caption{Reproduction of Studies on FB15K-237 where \textbf{pub} refers to published results, \textbf{R} to results based on the realistic ranking, \textbf{O} to results based on the optimistic ranking, and \textbf{P} to results based on the pessimistic ranking. 
    For published results, there are two additional rank types, \textbf{U} for undefined due to missing official implementation and \textbf{ND} for non-deterministic.
    We only show the results of the optimistic and pessimistic ranking in case they differ from the realistic ranking.}
    \label{tab:rps_fb15k237}
    \input{tables/reproducibility/fb15k237_table}
\end{table}


\begin{table}[H]
    \centering
    \caption{Reproduction of Studies on WN18 where \textbf{pub} refers to published results, \textbf{R} to results based on the realistic ranking, \textbf{O} to results based on the optimistic ranking, and \textbf{P} to results based on the pessimistic ranking.
    For published results, there are two additional rank types, \textbf{U} for undefined due to missing official implementation and \textbf{ND} for non-deterministic.
    We only show the results of the optimistic and pessimistic ranking in case they differ from the realistic ranking.\tnote{a}}
    \label{tab:rps_wn18}
    \input{tables/reproducibility/wn18_table}
\end{table}


\begin{table}[H]
    \centering
    \caption{Reproduction of Studies on WN18RR where \textbf{pub} refers to published results, \textbf{R} to results based on the realistic ranking, \textbf{O} to results based on the optimistic ranking, and \textbf{P} to results based on the pessimistic ranking.
    For published results, there are two additional rank types, \textbf{U} for undefined due to missing official implementation and \textbf{ND} for non-deterministic.
    We only show the results of the optimistic and pessimistic ranking in case they differ from the realistic ranking.}
    \label{tab:rps_wn18rr}
    \begin{threeparttable}
    \input{tables/reproducibility/wn18rr_table}
    \begin{tablenotes}
        \item[a] For MuRE, we obtained non-finite loss values while training on WN18RR with the setting defined in~\cite{DBLP:conf/nips/BalazevicAH19}. This might be explained by the fact that the specified learning rate of 50 is comparably large.
        In our benchmarking study, we show that we can outperform the published results with a different setting (Section~\ref{benchmarking_results_wn18rr}).
    \end{tablenotes}
\end{threeparttable}
\end{table}


\begin{table}[H]
    \centering
    \caption{%
    Model sizes in bytes for the best reported configurations studied for the the reproducibility study.%
    }
    \label{tab:repro_size}
\begin{tabular}{lrrrr}
\toprule
Dataset &     FB15K &  FB15K-237 &      WN18 &    WN18RR \\
Model    &           &           &           &           \\
\midrule
ComplEx  &   26.1 MB &         - &   49.2 MB &         - \\
ConvE    &   22.5 MB &   20.3 MB &   41.2 MB &   40.9 MB \\
ConvKB   &         - &    5.9 MB &         - &    8.2 MB \\
DistMult &    6.5 MB &         - &   16.4 MB &         - \\
HolE     &    9.8 MB &         - &   24.6 MB &         - \\
KG2E     &    6.5 MB &         - &   16.4 MB &         - \\
RotatE   &  130.4 MB &  117.9 MB &  163.8 MB &  162.3 MB \\
SimplE   &   26.1 MB &         - &   65.5 MB &         - \\
TransD   &    6.5 MB &         - &   16.4 MB &         - \\
TransE   &    3.3 MB &         - &    3.3 MB &         - \\
TransH   &    7.1 MB &         - &    8.2 MB &         - \\
TransR   &   16.7 MB &         - &    8.4 MB &         - \\
TuckER   &   46.1 MB &         - &   37.6 MB &         - \\
\bottomrule
\end{tabular}
\end{table}

==> tables/tables_main.tex <==

\begin{table}[t]
\centering
\caption{Investigated interaction models~\cite{Nickel2016} and their required number of parameters. $k$ corresponds to the number of neurons in the hidden layer, $n_f$ to the number of convolutional kernels, $k_r$ and $k_c$ to the height and width of the convolutional kernels.}\label{tab:supported_kge_models}
\begin{threeparttable}
\begin{tabular}{ll}
\toprule
Model & Parameters\\
\midrule
ComplEx\tnote{a}       & $|\mathcal{E}| 2d + |\mathcal{R}| 2d$ \\
ConvE\tnote{b}          & \begin{tabular}[c]{@{}l@{}l@{}l@{}}$|\mathcal{E}|d + |\mathcal{R}|d + d + n_f k_r k_c + 2 + 2n_f + 2d$ \\ $+ (h-k_r+1) (w-k_c+1)n_f d  +|\mathcal{E}|$\end{tabular} \\
ConvKB      & $|\mathcal{E}| d + |\mathcal{R}| d + n_f (d + 4) + 1$ \\
DistMult          & $|\mathcal{E}|  d  + |\mathcal{R}| d$ \\
ER-MLP             & $|\mathcal{E}| d + |\mathcal{R}| d + k(3d + 2) + 1$ \\
HolE             & $|\mathcal{E}|  d  + |\mathcal{R}| d$ \\
KG2E         & $|\mathcal{E}|2d + 2 |\mathcal{R}|d$ \\
MuRE        & $|\mathcal{E}| (d + 2) + 3 |\mathcal{R}|d$ \\
NTN     & $|\mathcal{E}| d + |\mathcal{R}|k(d^2 + 2 d + 2)$ \\
ProjE          & $|\mathcal{E}| d + |\mathcal{R}| d + 3d + 1$ \\
QuatE\tnote{c}           & $|\mathcal{E}|  4d  + |\mathcal{R}|  4d$ \\
RESCAL           & $|\mathcal{E}|  d  + |\mathcal{R}|  d^2$ \\
RotatE\tnote{a}    & $|\mathcal{E}| 2d + |\mathcal{R}| d$ \\
\ac{se}      & $|\mathcal{E}| d + 2 |\mathcal{R}| d^2$ \\
SimplE     & $|\mathcal{E}| 2d + 2|\mathcal{R}|d$ \\
TransE  & $|\mathcal{E}|  d  + |\mathcal{R}|  d$ \\
TransH    & $|\mathcal{E}|  d  +  2 |\mathcal{R}| d$ \\
TransR     & $|\mathcal{E}|  d_e +  |\mathcal{R}| d_r + d_e d_r$ \\
\ac{um}     & $|\mathcal{E}|d$ \\
TuckER & $|\mathcal{E}| d_e  + |\mathcal{R}| d_r + d_e^2 d_r + 4d_e$ \\
\bottomrule
\end{tabular}
\begin{tablenotes}
        \item[a] $2 d$, because of complex valued vectors, i.e.\ imaginary and real part of a number.
        \item[b] $w$ and $h$ correspond to the height and weight of the reshaped input.
        \item[c] $4 d$, because of hyper-complex valued (quaternion) vectors, i.e.\ a real part and three imaginary parts of a quaternion.
    \end{tablenotes}
\end{threeparttable}
\end{table}


\begin{table}[t]
\caption{Denotes for each proposed model whether results have been reported for FB15K, WN18, or their alterations.
Furthermore, it indicates whether an official implementation exists where P corresponds to a PyTorch based implementation, T to a TensorFlow based implementation, and O to other implementations.
A green background indicates that the full experimental setup was available. The models highlighted with * where included in the reproducibility study.}
\label{fig:overview_model_dataset}
\begin{threeparttable}
\begin{tabular}{lccccc}
\toprule
Model & Code & FB15K & FB15K-237 & WN18 & WN18RR\\
\midrule
ComplEx* & O &\cellcolor[HTML]{ADF7AD}\checkmark &    &  \cellcolor[HTML]{ADF7AD}\checkmark    &   \\
ConvE* &  P & \checkmark & \checkmark & \checkmark  &  \checkmark \\
ConvKB* & T & & \checkmark &     & \checkmark  \\
DistMult* &- & \cellcolor[HTML]{ADF7AD}\checkmark &   & \cellcolor[HTML]{ADF7AD}\checkmark &   \\
ER-MLP &- & & & &      \\
HolE*  & O &\checkmark& &\checkmark&     \\
KG2E* &- &\cellcolor[HTML]{ADF7AD}\checkmark& &\cellcolor[HTML]{ADF7AD}\checkmark&     \\
MuRE* &P &  & \cellcolor[HTML]{ADF7AD}\checkmark &  &  \cellcolor[HTML]{ADF7AD}\checkmark \\
\ac{ntn} &- & & & &       \\
ProjE &T &\cellcolor[HTML]{ADF7AD}\checkmark& & \cellcolor[HTML]{ADF7AD}\checkmark &       \\
QuatE*\tnote{a}  & P & \cellcolor[HTML]{ADF7AD}\checkmark & \cellcolor[HTML]{ADF7AD}\checkmark & \cellcolor[HTML]{ADF7AD}\checkmark  &  \cellcolor[HTML]{ADF7AD}\checkmark \\
\ac{um}  &- & & & &   \\
RESCAL & O & & & &      \\
RotatE* & P & \checkmark & \checkmark & \checkmark & \checkmark\\
\ac{se} & O & & & &       \\
SimplE*  &T, P &\cellcolor[HTML]{ADF7AD}\checkmark& &\cellcolor[HTML]{ADF7AD}\checkmark&     \\
TransD* & - &\cellcolor[HTML]{ADF7AD}\checkmark& &\cellcolor[HTML]{ADF7AD}\checkmark&    \\
TransE* & O &\checkmark& &\checkmark& \\
TransH* & - &\cellcolor[HTML]{ADF7AD}\checkmark& &\cellcolor[HTML]{ADF7AD}\checkmark&  \\
TransR* &O &\cellcolor[HTML]{ADF7AD}\checkmark& &\cellcolor[HTML]{ADF7AD}\checkmark&   \\
TuckER*  & P & \cellcolor[HTML]{ADF7AD}\checkmark & \cellcolor[HTML]{ADF7AD}\checkmark & \cellcolor[HTML]{ADF7AD}\checkmark  &  \cellcolor[HTML]{ADF7AD}\checkmark \\
\ac{um}  &- & & & &   \\
\bottomrule
\end{tabular}%
\begin{tablenotes}
        \item[a] Code is based on the framework OpenKE~\url{https://github.com/thunlp/OpenKE}.
    \end{tablenotes}
\end{threeparttable}
\end{table}

\begin{table}[t]
    \centering
    \caption{Hyper-Parameter Ranges for Ablation Experiments}
    \label{tab:hpo_params}
    \begin{threeparttable}
    \begin{tabular}{lll}
        \toprule
        & Hyper-Parameter     & Range  \\
        \midrule
        \multirow{7}{*}{\rotatebox[origin=c]{90}{Shared}}
        & Embedding-Dimension & \{64,128,256\} \\
        & Initialization & \{Xavier\} \\
        & Optimizers\tnote{a} & \{Adam, Adadelta\} \\
        & Learning Rate (log scale) & [0.001, 0.1) \\
        & Batch Size\tnote{b} & \{128, 256, 512\} \\
        & Model inverse relations & \{Yes, No\} \\
        & Epochs & 1,000 \\
        \midrule
        \multirow{5}{*}{\rotatebox[origin=c]{90}{\ac{slcwa}}}
        & Loss & \{\ac{bcel}, \ac{mrl}, \ac{nssal}, \ac{spl}\} \\
        & Margin for \ac{mrl} & \{0.5, 1.5, ... , 9.5\} \\
        & Margin for \ac{nssal} & \{1, 3, 5, ... , 29\} \\
        & ADVT for \ac{nssal} & \{0.1, 0.2, ... , 1.0\} \\
        & Number of Negatives\tnote{c} & \{1, 2, ... , 100\} \\
         \midrule
         \multirow{3}{*}{\rotatebox{90}{\ac{lcwa}}}
         & Loss & \{\ac{bcel}, \ac{cel}, \ac{spl}\} \\
         & Label Smoothing (log scale) & [0.001, 1.0)\\
         &&\\
        \bottomrule
    \end{tabular}
    \begin{tablenotes}
        \item[a] For Kinships, we evaluated Adam and Adadelta, and for the remaining datasets we sticked to Adam since it performed almost in every experiment at least equally good as Adadelta and in many experiments significantly better.
        \item[b] For YAGO3-10, the batch-size has been sampled from the set \{1024, 2048, 2096, 8192\}.
        \item[c] For YAGO3-10, the number of negative triples per each each positive has been sampled from the set \{1, 2, ..., 50\}.
    \end{tablenotes}
\end{threeparttable}
\end{table}{}

\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.2}
    \caption{Evaluation statistics}
    \begin{tabular}{lr}
        \toprule 
        Metric & Value \\
        \midrule 
         Datasets & 4 \\
         Interaction Models & 21 \\
         Training approaches & 2 \\
         Loss Functions & 5 \\
         Negative Samplers & 1 \\
         Optimizers & 2 \\
         Ablation Studies & 1,207 \\
         Number of Experiments & 73,683 \\
         Compute Time (hours) & 24,804 \\
         \bottomrule
    \end{tabular}
    \label{tab:eval_stats}
\end{table}
